Radial velocity signatures of Zeeman broadening

Stellar activity signatures such as spots and plage can significantly limit the search for extrasolar planets. Current models of activity-induced radial velocity (RV) signals focused on the impact of temperature contrast in spots predicting the signal to diminish toward longer wavelengths. On the other hand, the relative importance of the Zeeman effect on RV measurements should grow with wavelength, because the Zeeman displacement itself grows with \lambda, and because a magnetic and cool spot contributes more to the total flux at longer wavelengths. We model the impact of active regions on stellar RV measurements including both temperature contrast in spots and Zeeman line broadening. We calculate stellar line profiles using polarized radiative transfer models including atomic and molecular Zeeman splitting from 0.5 to 2.3\mum. Our results show that the amplitude of the RV signal caused by the Zeeman effect alone can be comparable to that caused by temperature contrast. Furthermore, the RV signal caused by cool and magnetic spots increases with wavelength. We also calculate the RV signal due to variations in average magnetic field strength from one observation to the next, but find it unlikely that this can significantly influence the search for extrasolar planets. As an example, we derive the RV amplitude of the active M dwarf AD Leo as a function of wavelength using data from the HARPS spectrograph. The RV signal does not diminish at longer wavelengths but shows evidence for the opposite behavior. We conclude that the RV signal of active stars does not vanish at longer wavelength but sensitively depends on the combination of spot temperature and magnetic field; in active low-mass stars, it is even likely to grow with wavelength.

==> PaxHeaders.16679/RadVelZeeman3.tex <==
20 atime=1358162918
20 ctime=1358162918

